Zero-1-to-G: Taming Pretrained 2D Diffusion Model for Direct 3D Generation

Recent advances in 2D image generation have achieved remarkable quality,largely driven by the capacity of diffusion models and the availability of large-scale datasets. However, direct 3D generation is still constrained by the scarcity and lower fidelity of 3D datasets. In this paper, we introduce Zero-1-to-G, a novel approach that addresses this problem by enabling direct single-view generation on Gaussian splats using pretrained 2D diffusion models. Our key insight is that Gaussian splats, a 3D representation, can be decomposed into multi-view images encoding different attributes. This reframes the challenging task of direct 3D generation within a 2D diffusion framework, allowing us to leverage the rich priors of pretrained 2D diffusion models. To incorporate 3D awareness, we introduce cross-view and cross-attribute attention layers, which capture complex correlations and enforce 3D consistency across generated splats. This makes Zero-1-to-G the first direct image-to-3D generative model to effectively utilize pretrained 2D diffusion priors, enabling efficient training and improved generalization to unseen objects. Extensive experiments on both synthetic and in-the-wild datasets demonstrate superior performance in 3D object generation, offering a new approach to high-quality 3D generation.

==> sec/0_abstract.tex <==
\begin{abstract}
% The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
% Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
% The abstract is to be in 10-point, single-spaced type.
% Leave two blank lines after the Abstract, then begin the main text.
% Look at previous \confName abstracts to get a feel for style and length.

We present \papername, a method to generate 3D Gaussian representation using 2D diffusion priors through the decomposition of Gaussian splatter images. 
While diffusion model on 2D images has shown impressive generation quality,
training a 3D diffusion model can hardly achieve comparable rendering results as a 2D diffusion model
due to the lack of a large 3D dataset. 
Our key insight is to utilize the rich 2D diffusion prior in the 3D diffusion model, by decomposing 3D Gaussian splatter images into multiple 3-channel images that can be modeled by a 2D diffusion model. 
Our experiment shows that these decomposed triplet images are well modeled in the distribution of the 2D diffusion model, therefore unleashing the great potential of 2D diffusion prior benefit from a large amount of training data, enabling efficient 3D diffusion model training with less data. 

\end{abstract}
